Standard model extensions for PV electron scattering, g-2, EDM: Overview

I review how various extensions of the Standard Model, in particular supersymmetry and extra neutral gauge bosons, may affect low energy observables, including parity-violating electron scattering and related observables, as well as electric and magnetic dipole moments.

==> PaxHeader/erler.tex <==
18 uid=1301562787
20 ctime=1319507932
20 atime=1319640226
24 SCHILY.dev=754974725
26 SCHILY.ino=13076253964
18 SCHILY.nlink=1

